Enforcing Architectural Styles in Presence of Unexpected Distributed Reconfigurations

Architectural Design Rewriting (ADR, for short) is a rule-based formal framework for modelling the evolution of architectures of distributed systems. Rules allow ADR graphs to be refined. After equipping ADR with a simple logic, we equip rules with pre- and post-conditions; the former constraints the applicability of the rules while the later specifies properties of the resulting graphs. We give an algorithm to compute the weakest pre-condition out of a rule and its post-condition. On top of this algorithm, we design a simple methodology that allows us to select which rules can be applied at the architectural level to reconfigure a system so to regain its architectural style when it becomes compromised by unexpected run-time reconfigurations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{M. Carbone, I. Lanese, A. Silva, A. Sokolova (Eds.):\\
5th Interaction and Concurrency Experience (ICE'12).\\
EPTCS 104, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.104.7}{10.4204/EPTCS.104.7}}
\pdfoutput=1

